Faster and Better Quantum Software Testing through Specification Reduction and Projective Measurements

Quantum computing promises polynomial and exponential speedups in many domains, such as unstructured search and prime number factoring. However, quantum programs yield probabilistic outputs from exponentially growing distributions and are vulnerable to quantum-specific faults. Existing quantum software testing (QST) approaches treat quantum superpositions as classical distributions. This leads to two major limitations when applied to quantum programs: (1) an exponentially growing sample space distribution and (2) failing to detect quantum-specific faults such as phase flips. To overcome these limitations, we introduce a QST approach, which applies a reduction algorithm to a quantum program specification. The reduced specification alleviates the limitations (1) by enabling faster sampling through quantum parallelism and (2) by performing projective measurements in the mixed Hadamard basis. Our evaluation of 143 quantum programs across four categories demonstrates significant improvements in test runtimes and fault detection with our reduction approach. Average test runtimes improved from 169.9s to 11.8s, with notable enhancements in programs with large circuit depths (383.1s to 33.4s) and large program specifications (464.8s to 7.7s). Furthermore, our approach increases mutation scores from 54.5% to 74.7%, effectively detecting phase flip faults that non-reduced specifications miss. These results underline our approach's importance to improve QST efficiency and effectiveness.

==> TikzCircuit/circuit_background.tex <==
% variables for adjusting coordinates of text in tikzpicture for the quantum circuit 
\pgfmathsetmacro{\xcoordinateVar}{5.1}
\pgfmathsetmacro{\ycoordinatebVar}{4.8}


\begin{figure}[tbp]
  \centering
  \hspace*{2em} % Adjust the horizontal spacing as needed
\Qcircuit @C=1em @R=.7em {
  \lstick{\ket{x_0}} & \multigate{4}{Main\;Program\; \mathcal{U}} & \multigate{4}{\mathcal{T}} & \qw & \meter \\
  \lstick{\ket{x_1}} & \ghost{Main\;Program\; \mathcal{U}} & \ghost{\mathcal{B}} & \qw & \meter \\
  \lstick{\ket{x_2}} & \ghost{Main\;Program\; \mathcal{U}} & \ghost{\mathcal{B}} & \qw & \meter \\
  \lstick{\vdots}    & \ghost{Main\;Program\; \mathcal{U}} & \ghost{\mathcal{B}} & & \vdots \\
  \lstick{\ket{x_{n-1}}} & \ghost{Main\;Program\; \mathcal{U}} & \ghost{\mathcal{B}} & \qw & \meter \gategroup{1}{4}{5}{5}{.8em}{--} \\
}
  \begin{tikzpicture}[overlay]
      \node at (4.3-\xcoordinateVar , 2.9-\ycoordinatebVar) {$M$};
      \node at (0.2-\xcoordinateVar, 1.5-\ycoordinatebVar) {$\ket{\psi_{init}}$};
      \node at (0.2-\xcoordinateVar, 1.8-\ycoordinatebVar) {$\uparrow$};
      \node at (3.0-\xcoordinateVar, 1.5-\ycoordinatebVar) {$\ket{\psi_{final}}$};
      \node at (3.1-\xcoordinateVar, 1.8-\ycoordinatebVar) {$\uparrow$};
      \node at (5.3-\xcoordinateVar, 1.5-\ycoordinatebVar) {$O_m$};
      \node at (5.3-\xcoordinateVar, 1.8-\ycoordinatebVar) {$\uparrow$};
  \end{tikzpicture}
  \vspace{12pt} % Add more space above the caption
  \caption{Illustration of a quantum program under a projective measurement $\mathcal{T}M$.}
  \Description{Quantum program consisting of the initial state $\ket{\psi_{init}}$, main program $\mathcal{U}$ and the measurement M with respect to the basis $\mathcal{B}$. The measurement results in the output $O_m=\ket{m}$, a definite state of $0s$ and $1s$ that represents the basis states of the transformation $T_{\mathcal{B}}$. }
  \label{fig:quantum-circuit}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

